Motion Design Principles for Accessible Video-based Learning: Addressing Cognitive Challenges for Deaf and Hard of Hearing Learners

Deaf and Hard-of-Hearing (DHH) learners face unique challenges in video-based learning due to the complex interplay between visual and auditory information in videos. Traditional approaches to making video content accessible primarily focus on captioning, but these solutions often neglect the cognitive demands of processing both visual and textual information simultaneously. This paper introduces a set of \textit{Motion} design guidelines, aimed at mitigating these cognitive challenges and improving video learning experiences for DHH learners. Through a two-phase research, we identified five key challenges, including misaligned content and visual overload. We proposed five design principles accordingly. User study with 16 DHH participants showed that improving visual-audio relevance and guiding visual attention significantly enhances the learning experience by reducing physical demand, alleviating temporal pressure, and improving learning satisfaction. Our findings highlight the potential of Motion design to transform educational content for DHH learners, and we discuss implications for inclusive video learning tools.

==> backuptable.tex <==
\begin{table}[]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{lcclcclcclccl}
 &
  \multicolumn{2}{c}{Mental Demand} &
   &
  \multicolumn{2}{c}{Physical Demand} &
   &
  \multicolumn{2}{c}{Temporal Pressure} &
   &
  \multicolumn{2}{c}{Learning Satisfaction} &
   \\
 &
  Original &
  Revised &
   &
  Original &
  Revised &
   &
  Original &
  Revised &
   &
  Original &
  Revised &
   \\
Design Idea &
  Mean (SD) &
  Mean (SD) &
   &
  Mean (SD) &
  Mean (SD) &
   &
  Mean (SD) &
  Mean (SD) &
   &
  Mean (SD) &
  Mean (SD) &
   \\
D-Illustrate &
  \textbf{3.09 (2.17)} &
  \textbf{2.39 (1.93)} &
  \multicolumn{1}{c}{\textbf{*}} &
  \textbf{3.01 (2.18)} &
  \textbf{2.31 (2.10)} &
  \multicolumn{1}{c}{\textbf{*}} &
  \textbf{2.96 (2.11)} &
  \textbf{2.28 (1.75)} &
  \multicolumn{1}{c}{\textbf{*}} &
  \textbf{7.75 (2.23)} &
  \textbf{8.90 (2.12)} &
  \multicolumn{1}{c}{\textbf{***}} \\
D-Align &
  2.95 (2.11) &
  2.43 (1.91) &
   &
  \textbf{2.89 (2.26)} &
  \textbf{2.43 (2.02)} &
  \multicolumn{1}{c}{*} &
  \textbf{2.88 (1.96)} &
  \textbf{2.35 (1.87)} &
  \multicolumn{1}{c}{\textbf{*}} &
  \textbf{8.06 (2.25)} &
  \textbf{8.74 (2.14)} &
  \multicolumn{1}{c}{\textbf{*}} \\
D-Declutter &
  3.04 (1.98) &
  2.63 (2.11) &
   &
  3.27 (2.46) &
  2.67 (2.30) &
   &
  2.98 (2.10) &
  2.52 (2.03) &
   &
  \textbf{7.69 (2.25)} &
  \textbf{8.50 (2.12)} &
  \multicolumn{1}{c}{\textbf{*}} \\
D-Slowdown &
  2.81 (1.74) &
  2.63 (1.92) &
   &
  2.90 (2.13) &
  2.71 (2.21) &
   &
  2.92 (1.82) &
  2.81 (2.02) &
   &
  8.29 (1.98) &
  8.23 (2.20) &
   \\
\end{tabular}%
}
\caption{Si-New Table-Mean (SD) scores before and after applying each design idea, with significance indicators from mixed-effects models and Bonferroni-corrected tests.}
\end{table}

